Does complimentary information from multispectral imaging improve face presentation attack detection?

Presentation Attack Detection (PAD) has been extensively studied, particularly in the visible spectrum. With the advancement of sensing technology beyond the visible range, multispectral imaging has gained significant attention in this direction. We present PAD based on multispectral images constructed for eight different presentation artifacts resulted from three different artifact species. In this work, we introduce Face Presentation Attack Multispectral (FPAMS) database to demonstrate the significance of employing multispectral imaging. The goal of this work is to study complementary information that can be combined in two different ways (image fusion and score fusion) from multispectral imaging to improve the face PAD. The experimental evaluation results present an extensive qualitative analysis of 61650 sample multispectral images collected for bonafide and artifacts. The PAD based on the score fusion and image fusion method presents superior performance, demonstrating the significance of employing multispectral imaging to detect presentation artifacts.

==> reference.tex <==

@article{article,
	author = {Sharma, Deepika and Selwal, Arvind},
	year = {2023},
	month = {03},
	pages = {1-51},
	title = {A survey on face presentation attack detection mechanisms: hitherto and future perspectives},
	volume = {29},
	journal = {Multimedia Systems},
}

@manual{ISO-IEC-JTC-SC37-2013,
	Author = {{ISO/IEC JTC1 SC37 Biometrics}},
	Date-Added = {2016-05-23 15:12:04 +0000},
	Date-Modified = {2016-05-23 15:12:04 +0000},
	Month = March,
	Organization = {Testing and Reporting, International Organization for Standardization and International Electrotechnical Committee},
	Title = {ISO/IEC DIS 30107-3. Biometrics- Presentation Attack Detection - Part 3},
	Year = {August, 2016},
}

@ARTICLE{8714076,
	author={George, Anjith and Mostaani, Zohreh and Geissenbuhler, David and Nikisins, Olegs and Anjos, André and Marcel, Sébastien},
	journal={IEEE Transactions on Information Forensics and Security}, 
	title={Biometric Face Presentation Attack Detection With Multi-Channel Convolutional Neural Network}, 
	year={2020},
	volume={15},
	pages={42-55},
}

@misc{george2022comprehensive,
	title={A Comprehensive Evaluation on Multi-channel Biometric Face Presentation Attack Detection}, 
	author={Anjith George and David Geissbuhler and Sebastien Marcel},
	year={2022},
	eprint={2202.10286},
	archivePrefix={arXiv},
	primaryClass={cs.CV}
}

@Inbook{Bhattacharjee2019,
	author="Bhattacharjee, Sushil
	and Mohammadi, Amir
	and Anjos, Andr{\'e}
	and Marcel, S{\'e}bastien",
	editor="Marcel, S{\'e}bastien
	and Nixon, Mark S.
	and Fierrez, Julian
	and Evans, Nicholas",
	title="Recent Advances in Face Presentation Attack Detection",
	bookTitle="Handbook of Biometric Anti-Spoofing: Presentation Attack Detection",
	year="2019",
	publisher="Springer International Publishing",
	address="Cham",
	pages="207--228",
}

@INPROCEEDINGS{8311455,
	author={Raghavendra, R. and Vetrekar, Narayan and Raja, Kiran B. and Gad, R. S. and Busch, Christoph},
	booktitle={2018 IEEE 4th International Conference on Identity, Security, and Behavior Analysis (ISBA)}, 
	title={Robust gender classification using extended multi-spectral imaging by exploring the spectral angle mapper}, 
	year={2018},
	pages={1-8},
}

@INPROCEEDINGS{7738245,
	author={Vetrekar, N.T. and Raghavendra, R. and Gad, R.S.},
	booktitle={2016 IEEE International Conference on Imaging Systems and Techniques (IST)}, 
	title={Low-cost multi-spectral face imaging for robust face recognition}, 
	year={2016},
	pages={324-329},
}

@misc{Phd-toolbox,
	author    = "Vitomir Struc",
	title     = "PhD (Pretty helpful Development function for) face recognition toolbox",
	note      = "Software available at \url{http://luks.fe.uni-lj.si/sl/osebje/vitomir/face_tools/PhDface/}",
}

@INPROCEEDINGS{X.Zhu:face-detect-based-landmarks:CVPR:2012, 
	author={X. Zhu and D. Ramanan}, 
	booktitle={IEEE Conference on Computer Vision and Pattern Recognition}, 
	title={Face detection, pose estimation, and landmark localization in the wild}, 
	year={2012}, 
	pages={2879-2886}, 
	month={June},
	note={Software available at \url{https://www.ics.uci.edu/~xzhu/face/}},
}


@ARTICLE{1717463,
	author={Ahonen, T. and Hadid, A. and Pietikainen, M.},
	journal={IEEE Transactions on Pattern Analysis and Machine Intelligence}, 
	title={Face Description with Local Binary Patterns: Application to Face Recognition}, 
	year={2006},
	volume={28},
	number={12},
	pages={2037-2041},
	doi={10.1109/TPAMI.2006.244}
}

@INPROCEEDINGS{8014830,
	author={Raghavendra, R. and Raja, Kiran B. and Venkatesh, Sushma and Busch, Christoph},
	booktitle={2017 IEEE Conference on Computer Vision and Pattern Recognition Workshops (CVPRW)}, 
	title={Face Presentation Attack Detection by Exploring Spectral Signatures}, 
	year={2017},
	pages={672-679},
}

@misc{george2022comprehensive,
	title={A Comprehensive Evaluation on Multi-channel Biometric Face Presentation Attack Detection}, 
	author={Anjith George and David Geissbuhler and Sebastien Marcel},
	year={2022},
	eprint={2202.10286},
	archivePrefix={arXiv},
	primaryClass={cs.CV}
}

@ARTICLE{iet:content-journals,
	author = {Artur Costa‐Pazo},
	author = {Daniel Pérez‐Cabo},
	author = {David Jiménez‐Cabello},
	author = {José Luis Alba‐Castro},
	author = {Esteban Vazquez‐Fernandez},
	journal = {IET Biometrics},
	issue = {4},   
	volume = {10},
	year = {2021},
	month = {July},
	pages = {408-429(21)},
	publisher ={Institution of Engineering and Technology},
}




